Decentralized Optimization On Time-Varying Directed Graphs Under Communication Constraints

We consider the problem of decentralized optimization where a collection of agents, each having access to a local cost function, communicate over a time-varying directed network and aim to minimize the sum of those functions. In practice, the amount of information that can be exchanged between the agents is limited due to communication constraints. We propose a communication-efficient algorithm for decentralized convex optimization that rely on sparsification of local updates exchanged between neighboring agents in the network. In directed networks, message sparsification alters column-stochasticity -- a property that plays an important role in establishing convergence of decentralized learning tasks. We propose a decentralized optimization scheme that relies on local modification of mixing matrices, and show that it achieves $\mathcal{O}(\frac{\mathrm{ln}T}{\sqrt{T}})$ convergence rate in the considered settings. Experiments validate theoretical results and demonstrate efficacy of the proposed algorithm.

==> consensus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem Formulation}\label{sec21}
Suppose there are $n$ nodes in a network and that each of them keeps a local parameter vector. 
The average consensus problem is formalized as the computation $\Bar{\x}=\frac{1}{n}\sum_{i=1}^n \mathbf{x}_i$,
% \begin{equation}
% \Bar{\x}=\frac{1}{n}\sum_{i=1}^n \mathbf{x}_i,
% \end{equation}
where $\mathbf{x}_i \in \mathbb{R}^d$ is the parameter vector at node $i$. 
[Note that the average consensus 
problem is an instance of the general decentralized optimization problem \eqref{eq:problem}, where the local objective function at node $i$ is $f_i(\x)=\frac{1}{2}\|\x-\x_i \|^2$.] The goal of average consensus is that nodes of a network, whose communication is constrained by the network topology, reach the average of the initial local vectors.
Communication between the network's nodes is modeled by a directed time-varying graph. In particular, let $W_{in}^t$ (row-stochastic) and $W_{out}^t$ (column-stochastic) denote the in-neighbor and 
out-neighbor connectivity matrix at time $t$, respectively. That is, 
\begin{equation}
[W_{in}^t]_{ij}=\begin{cases}
>0, & j \in \mathcal{N}_{{in},i}^t \\
0, & \mathrm{otherwise}
\end{cases}, \qquad
[W_{out}^t]_{ij}=\begin{cases}
>0, & i \in \mathcal{N}_{out,j}^t \\
0, & \mathrm{otherwise}
\end{cases}
\end{equation}
% \begin{equation}
% [W_{in}^t]_{ij}=\begin{cases}
% >0, & j \in \mathcal{N}_{{in},i}^t \\
% 0, & \mathrm{otherwise}
% \end{cases} 
% \end{equation}
% \begin{equation}
% [W_{out}^t]_{ij}=\begin{cases}
% >0, & i \in \mathcal{N}_{out,j}^t \\
% 0, & \mathrm{otherwise}
% \end{cases}
% \end{equation}
where $\mathcal{N}_{{in},i}^t$ is the set of nodes that can send information to node $i$ (including $i$) and 
$\mathcal{N}_{out,j}^t$ is the set of nodes that can receive information from node $j$  (including $j$) at time 
$t$. We assume $W_{in}^t$ and $W_{out}^t$ are given and that both $\mathcal{N}_{{in},i}^t$ and 
$\mathcal{N}_{out,i}^t$ are known to node $i$. Note that a simple policy for designing $W^t_{in}$ and $W^t_{out}$ is to set
\begin{equation}\label{eq:Ws}
[W^t_{in}]_{ij} = 1/|\mathcal{N}^t_{in, i}|, \qquad [W^t_{out}]_{ij}= 1/|\mathcal{N}^t_{out, j}|.
\end{equation}
Given the topology of a graph, one can use the above connectivity matrices to construct the mixing matrix (as formally stated in Definition~1 in Section \ref{sec22}). Throughout the paper, we impose the condition that the constructed mixing matrices have non-zero spectral gaps. This is satisfied for a variety of network structures, e.g. when the union graph is jointly-connected\footnote{
We formally state and discuss joint connectivity in the appendix (Section \ref{app:A1}). As a preview, we assume that there exists $\mathcal{B}\geq1$ such that the union graph $\bigcup_{l=t}^{t+\mathcal{B}-1}\G_{l}$ is strongly-connected for all $t = k\mathcal{B}$, $k \in \mathcal{N}$. If $\mathcal{B}=1$, each instance of the graph is strongly-connected. Note that this is a more general assumption than the commonly used $\mathcal{B}$-bounded strong-connectivity (see, e.g. \cite{nedic2017achieving}) which requires strong connectivity of the aggregate graph $\bigcup_{l=t}^{t+\mathcal{B}-1}\G_{l}$ for all $t \geq 0$. 
}.

%The jointly-connected assumption that  above we impose implies that the graph is not required to be connected at each time step.

% Additionally, we assume the graph at each time step is 
% connected, i.e., there exists a directed path between each pair of nodes in the network.

We consider the limited bandwidth setting typical of practical networks 
and high-dimensional scenarios (i.e., the problems where the dimension $d$ of 
local parameters $\x_i$ is very large). In such settings, nodes in the network may reduce the size of communicated messages by employing {\it sparsification}, here denote by the operator $Q: \mathbb{R}^d \rightarrow \mathbb{R}^d$. Sparsification can be performed in two ways: (i) each node 
selects $k$ out of $d$ entries of a $d$-dimensional message and communicates only 
the selected entries; or (ii) each component of a $d$-dimensional message 
is selected to be communicated with probability $k/d$. The first approach imposes a hard communication constraint (i.e., exactly $k$ entries are communicated) while in the latter the number of communicated entries is $k$ on expectation. In both approaches, 
the probability of selecting a specific entry is $k/d$; in this paper, we adopt the former. 

Note that our proposed sparsification operator is biased, i.e., $\mathbb{E}[Q(\x)] \neq \x$, and that its variance is a function of the norm of its argument, i.e. $\mathbb{E}[\|Q(\x)-\x\|^2] \propto \|\x\|^2$. This stands in contrast to the majority of existing works on communication-efficient decentralized learning
(see, e.g. \cite{tang2018communication}). More recent works \cite{stich2018sparsified,koloskova2019decentralized,koloskova2019decentralizeda,taheriquantized}, do consider such biased compression operators. However, the results therein are established assuming static communication networks which is a more restrictive setting than the one considered in the current paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Communication-Efficient Average Consensus}\label{sec22}

A straightforward 
sparsification of messages exchanged by existing consensus methods, e.g. \cite{kempe2003gossip,cai2012average,cai2014average,nedic2014distributed}, does not lead to convergent schemes due to non-vanishing error terms that stem from the bias and variance properties of the compression operator. Note that the impact of sparsification on the entries of a message vector is akin to the impact of link failures, and could thus be captured in the structure of the connectivity matrices. To clarify this, we observe that the vector-valued consensus problem can be interpreted as consisting of $d$ individual scalar-valued average consensus tasks with weight matrices at time $t$, $\{W_{in,m}^t\}_{m=1}^d$ and $\{W_{out,m}^t\}_{m=1}^d$. For the entries that are sparsified, i.e., set to zero and not communicated, the corresponding weight matrices are no longer stochastic while the weight matrices of communicated entries remain stochastic. Hence, we propose to judiciously {\it re-normalize} the weight matrices $\{W_{in,m}^t\}_{m=1}^d$ and $\{W_{out,m}^t\}_{m=1}^d$ to ensure their row and column stochasticity. Note that the re-normalization of the $i\ts{th}$ row of $\{W_{in,m}^t\}_{m=1}^d$ ($j\ts{th}$ column of $\{W_{out,m}^t\}_{m=1}^d$) is performed by node $i$ (node $j$) in the network. Let $\{A_{m}^t\}_{m=1}^d$ and $\{B_{m}^t\}_{m=1}^d$ denote the weight matrices obtained after normalizing $\{W_{in,m}^t\}_{m=1}^d$ and $\{W_{out,m}^t\}_{m=1}^d$, respectively. To define the normalization rule, we first need to specify the sparsification operation, discussed next.

Following the work of \cite{cai2012average} on consensus over static directed graphs, for each node we define an auxiliary variable $\mathbf{y}_i\in \mathbb{R}^d$ to aid in formalization of the proposed communication-efficient consensus scheme. This so-called surplus vector tracks local state vector variations over consecutive time steps, and ultimately guarantees convergence to the average consensus state. 
%{\color{blue}{I cannot introduce the update of surplus vector before the definition of the mixing matrix. However, I want to include some motivation for surplus vector when it is first introduced. I also added the elementwise update after \eqref{eq:update_consensus} and the state vector variation refers to the second term in \eqref{update_consensus_y}. }}
At time $t$, node $i$ sends its state vector $\mathbf{x}_i^t$ and the surplus vector $\mathbf{y}_i^t$ to its out-neighbors. To simplify the notation, let us introduce $\mathbf{z}_i^t \in \mathbb{R}^d$ defined as
\begin{equation}\label{eq:zdef}
\mathbf{z}_i^t = \begin{cases}
\mathbf{x}_i^t, & i \in \left\{1, ..., n \right\} \\
\mathbf{y}_{i-n}^t, & i \in \left\{n+1, ..., 2n \right\},
\end{cases}
\end{equation}
representing messages communicated between the nodes of the network. 
%{\color{blue}{Without surplus vectors, the communication of state vectors between nodes can be unidirectional in the time-varying directed network and this asymmetry prevents state vectors from reaching the average consensus state.}}
Sparsification of $\mathbf{x}_i^t$ (and, effectively, $\mathbf{y}_i^t$) is facilitated by applying the compression operator $Q(\cdot)$ to $\mathbf{z}_i^t$; the result is denoted by $Q(\mathbf{z}_i^t)$. Let $[Q({\z}_{i}^t)]_m$ denote the $m\ts{th}$ entry of $Q(\mathbf{z}_i^t)$. We can now formalize the normalization procedure by defining the weight matrix
\begin{equation}\label{eq:normA}
[A^t_m]_{ij}=\begin{cases}
\frac{[W^t_{in, m}]_{ij}}{\sum_{j\in\mathcal{S}_m^t(i,j)} [W^t_{in, m}]_{ij}} & \text{if } j\in\mathcal{S}_m^t(i,j)\\
0 & \mathrm{otherwise},
\end{cases}
\end{equation}
where $\mathcal{S}_m^t(i,j) := \{j|j\in\mathcal{N}^t_{in,i},[Q({\z}_{j}^t)]_m \neq 0\}\cup\{i\}$. Similarly, the weight matrix $B^t_m$ is obtained as
\begin{equation}\label{eq:normB}
[B^t_m]_{ij}=\begin{cases}
\frac{[W^t_{out, m}]_{ij}}{\sum_{i\in\mathcal{T}_m^t(i,j)} [W^t_{out, m}]_{ij}} & \text{if } i\in\mathcal{T}_m^t(i,j)\\
0 & \mathrm{otherwise},
\end{cases}
\end{equation}
where $\mathcal{T}_m^t(i,j) := \{i|i\in\mathcal{N}^t_{out,j},[Q({\z}_{i}^t)]_m \neq 0\}\cup\{j\}$.

To derive a compact consensus update rule, we first need to define the {\it mixing matrix} of a directed network with sparsified messages. 

\begin{definition}
The $m\ts{th}$ mixing matrix at time $t$ of a time-varying directed network with sparsified messages, $\Bar{M}_m^t \in \mathbb{R}^{2n \times 2n}$, is a matrix with column sum equal to $1$ and eigenvalues $1=|\lambda_1(\Bar{M}_m^t)| = |\lambda_2(\Bar{M}_m^t)| \geq |\lambda_3(\Bar{M}_m^t)| \geq \cdots |\lambda_{2n}(\Bar{M}_m^t)|$ that is constructed from the current network topology as
\begin{equation}\label{matrixdefbar}
\Bar{M}_m^t=\left[\begin{matrix}
   A_m^t & \mathbf{0} \\
   I-A_m^t & B_m^t \\
  \end{matrix}
\right],
\end{equation}
where $A_m^t$ and $B_m^t$ represent the $m\ts{th}$ normalized in-neighbor and out-neighbor connectivity matrices at time $t$, respectively. 
\end{definition}

Having defined $\mathbf{z}_i^t$ and $\bar{M}_m^t$ in \eqref{eq:zdef} and \eqref{matrixdefbar}, respectively, we now state a recursive update for $\mathbf{z}_i^t$ in the communication-efficient average consensus algorithm,
\begin{equation}\label{eq:update_consensus}
\begin{aligned}
z_{im}^{t+1}& = \sum_{j=1}^{2n}[\bar{M}^t_m]_{ij} [Q(\z_{j}^t)]_m  + \mathbbm{1}_{\left\{t \mod \mathcal{B} = \mathcal{B}-1\right\}} \epsilon [F]_{ij} z_{jm}^{\mathcal{B} \lfloor t/\mathcal{B} \rfloor},
\end{aligned}
\end{equation}
where $F =\left[ \begin{matrix} \mathbf{0} & I \\
\mathbf{0} & -I 
\end{matrix} \right]$ and $m$ denotes a coordinate index. Note that \eqref{eq:update_consensus} implies the following element-wise update rules for state and surplus vectors, respectively:
\begin{equation}\label{update_consensus_x}
\begin{aligned}
    x_{im}^{t+1} & = \sum_{j=1}^{n}[A_m^t]_{ij}[Q(\x_j^t)]_m + \mathbbm{1}_{\left\{t\mod \mathcal{B} = \mathcal{B}-1\right\}} \epsilon  y_{im}^{\mathcal{B} \lfloor t/\mathcal{B} \rfloor} 
\end{aligned}
\end{equation}
\begin{equation}\label{update_consensus_y}
\begin{aligned}
    y_{im}^{t+1} & = \sum_{j=1}^{n}[B_m^t]_{ij}[Q(\y_j^t)]_m   - (x_{im}^{t+1} - x_{im}^t). 
\end{aligned}
\end{equation}

As seen in (\ref{eq:update_consensus}), vectors $\z_i^t$ (which contain $\x_i^t$, objects to be averaged) are updated in a straightforward manner via sparsification and multiplication with the mixing matrix at all times $t$ except those that satisfy
\begin{equation}\label{eq:mod}
    t \mod \mathcal{B} = \mathcal{B}-1.
\end{equation}
In particular, when (\ref{eq:mod}) holds, vectors $\z_i^{\mathcal{B}\lfloor t/\mathcal{B} \rfloor}$, stored at time $\mathcal{B}\lfloor t/\mathcal{B} \rfloor$, are also used to update $\z_i^t$.\footnote{Note that $F$ has all-zero matrices for its $(1, 1)$ and $(2, 1)$ blocks and thus we only need to store $\z_i^{\mathcal{B}\lfloor t/\mathcal{B} \rfloor}$ (equivalently, $\y_{i-n}^{\mathcal{B}\lfloor t/\mathcal{B} \rfloor}$), where $n+1 \leq i \leq 2n$.}
The use of the stored vectors is motivated by an observation that $\Bar{M}_m^t$ may have spectral gap (i.e., the difference between the moduli of its largest two eigenvalues) equal to zero; this is undesirable since for such mixing matrices we are unable to guarantee convergence of the consensus algorithms. However, for a judiciously chosen perturbation parameter $\epsilon$, which determines
to which extent $\sum_{j=1}^{2n}[F]_{ij} z_{jm}^{\mathcal{B} \lfloor t/\mathcal{B} \rfloor}$ affects the update, we can ensure a nonzero spectral gap of the product of $\mathcal{B}$ consecutive mixing matrices starting from $t = k\mathcal{B}$. The described average consensus procedure is formalized as Algorithm \ref{alg:A}. 

Note that Algorithm \ref{alg:A} requires each node in the network to store local vectors of size $3d$, including the current state vector, current surplus vector, and past surplus vector. While the current state vector and current surplus vector may be communicated to the neighboring nodes, past surplus vectors are only used locally to add local perturbations at the time steps satisfying \eqref{eq:mod}. 

It is also worth pointing out that the columns of $\bar{M}_m^t$ sum up to one. However, $\bar{M}_m^t$ is not column-stochastic as it has negative entries. This is in contrast to the consensus problems over undirected graphs where the mixing matrix is doubly stochastic \cite{xiao2004fast,koloskova2019decentralized}. 

We further note that when $\mathcal{B} = 1$, the problem can be reduced to the special case of networks that are strongly connected at all time steps. In this case, we can represent the mixing matrix in the compact form
\begin{equation}\label{matrixdef}
M_m^t=\left[\begin{matrix}
   A_m^t & \epsilon I \\
   I-A_m^t & B_m^t-\epsilon I \\
  \end{matrix}
\right].
\end{equation}
Consequently, the recursive expression for $\z_i^t$ can be stated as
\begin{equation}\label{eq:update}
z_{im}^{t+1}=\sum_{j=1}^{2n}[M^t_m]_{ij} [Q(\z_{j}^t)]_m.
\end{equation}

% \begin{comment}
% \begin{definition}
% The $m\ts{th}$ mixing matrix in a time-varying directed network with sparsified messages at iteration $t$, $M_m^t \in \mathbb{R}^{2n \times 2n}$, is a column-stochastic matrix with eigenvalues $1=|\lambda_1(M_m^t)|\geq|\lambda_2(M_m^t)| \geq |\lambda_3(M_m^t)| \geq \cdots |\lambda_{2n}(M_m^t)|$, that is constructed from the current network topology as
% \begin{equation}\label{matrixdef}
% M_m^t=\left[\begin{matrix}
%   A_m^t & \epsilon I \\
%   I-A_m^t & B_m^t-\epsilon I \\
%   \end{matrix}
% \right],
% \end{equation}
% where $A_m^t$ and $B_m^t$ represent the $m\ts{th}$ normalized in-neighbor and out-neighbor connectivity matrices at time $t$, respectively, and $\epsilon \in (0, 1)$ is a parameter of the consensus algorithm. 
% \end{definition}

% The mixing matrix $M_m^t$ can be thought of as being a perturbed version of the matrix 
% \begin{equation}\label{matrixdefM}
% \Bar{M}_m^t=\left[\begin{matrix}
%   A_m^t & \mathbf{0} \\
%   I-A_m^t & B_m^t \\
%   \end{matrix}
% \right].
% \end{equation}
% \end{comment}

% \begin{comment}
% \begin{remark}
% It is worth noting that the columns of $M_m^t$ sum to one. However, $M_m^t$ is not column-stochastic as it has negative entries. This is in contrast to consensus problems over undirected graphs where the mixing matrix is double-stochastic \cite{xiao2004fast,koloskova2019decentralized}.

% Given the definitions of $\mathbf{z}_i^t$ and $M_m^t$, we can state the recursive expression for $\mathbf{z}_i^t$ as
% \begin{equation}\label{eq:update}
% z_{im}^{t+1}=\sum_{j=1}^{2n}[M^t_m]_{ij} [Q(\z_{j}^t)]_m.
% \end{equation}
% \end{remark}
% \end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Analysis}
Here we analyze Algorithm \ref{alg:A} and show that it achieves linear convergence rate.
%, thus matching the convergence rate of methods which do not sparsify messages. 
Before starting the analysis, it is convenient to denote the product of a sequence of time-varying matrices as 
\begin{equation}
 \bar{M}_m(T:s) = \bar{M}_m^{T} \bar{M}_m^{T-1} \cdots \bar{M}_m^s,   
\end{equation}
where the superscript is the time index and the subscript is the coordinate index. We will also find it convenient to introduce
\begin{equation}\label{mproduct}
M_m((k+1)\mathcal{B}-1:k\mathcal{B}) = \bar{M}_m((k+1)\mathcal{B}-1:k\mathcal{B}) + \epsilon F, \end{equation}
and
\begin{equation}
\begin{aligned}
M_m(t:k_1\mathcal{B})
= \bar{M}_m(t:k_2\mathcal{B})M_m(k_2\mathcal{B}-1:(k_2-1)\mathcal{B}) \cdots M_m((k_1+1)\mathcal{B}-1:k_1\mathcal{B}),
\end{aligned}
\end{equation}
where $k_2\mathcal{B} \leq t < (k_2+1)\mathcal{B}-1$ and $k_1, k_2 \in \mathcal{N}, k_1 \leq k_2$. Note that
$M_m((k+1)\mathcal{B}-1:k\mathcal{B})$ is formed by adding a perturbation matrix $\epsilon F $ to the product of mixing matrices $\bar{M}_m((k+1)\mathcal{B}-1:k\mathcal{B})$.


We proceed by stating assumptions about properties of the graph and network connectivity matrices.


\begin{assumption}\label{assumption0}
The product of consecutive mixing matrices $M_m((k+1)\mathcal{B}-1:k\mathcal{B})$ has a non-zero spectral gap for all $0 < \epsilon < \epsilon_0$, where $\epsilon_0>0$, $k \geq 0$ and $1 \leq m \leq d$.% (see Lemma \ref{lemma0}).
\end{assumption}

This assumption is readily satisfied for a variety of graph structures. In Appendix \ref{app:A}, we relate Assumption~1 to the graph structure and provide exact expressions for $\epsilon_0$ for graphs strongly connected at each time step as well as those jointly connected over $\mathcal{B}$ time steps.

\begin{assumption}\label{assumption2}
 For any fixed $\epsilon \in (0,1)$, the set of all possible mixing matrices $\{\bar{M}_m^t\}$ is finite.
 \end{assumption}
 
 Assumption \ref{assumption2} states that after taking into account the effect of randomly sparsified messages on the normalized weight matrices $A_m^t$ and $B_m^t$ and, in turn, the mixing matrix $\bar{M}_m^t$, the set of all possible mixing matrices is finite. It is straightforward to verify that Assumption \ref{assumption2} holds for the weight matrices in \eqref{eq:Ws}.

\begin{lemma}\label{lemma0}
Suppose that Assumptions \ref{assumption0} and \ref{assumption2} hold. 
There exists $\epsilon_0 >0$ such that if $\epsilon \in (0, \epsilon_0)$
then for all $m = 1, \cdots, d$ the following statements hold.
 
\begin{enumerate}[(a)]
\item The spectral norm of 
$M_m((k+1)\mathcal{B}-1:k\mathcal{B})$ satisfies
\begin{equation}
\begin{aligned}
\rho(M_m((k+1)\mathcal{B}-1:k\mathcal{B})) - \frac{1}{n}[\mathbf{1}^T \ \mathbf{0}^T]^T[\mathbf{1}^T \  \mathbf{1}^T])  = \sigma <1
     \end{aligned}
%     \rho(\bar{M}((s+1)\mathcal{B}-1:s\mathcal{B}))+\epsilon F - \frac{1}{n}[\mathbf{1}^T \ \mathbf{0}^T]^T[\mathbf{1}^T \  \mathbf{1}^T]) = \sigma <1
     \end{equation}
     $\forall k \in \mathcal{N}$.
\item 
There exists $\Gamma = \sqrt{2nd}>0$ such that
\begin{equation}
    \|
    M_m(n\mathcal{B}-1:0)-\frac{1}{n}[\mathbf{1}^T \ \mathbf{0}^T]^T[\mathbf{1}^T \  \mathbf{1}^T]\|_{\infty} \leq \Gamma \sigma^{n}.
    \end{equation}
 \end{enumerate}
 \end{lemma}

\begin{algorithm}[t]
\caption{Communication-sparsified consensus over jointly-connected graphs}
\label{alg:A}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} 
   $T$, % Time horizon
   $\mathbf{x}^0$, % Initial state
   $\mathbf{y}^0=\mathbf{0}$, % Initial y
   
\STATE {set $\mathbf{z}^0=[\mathbf{x}^0; \mathbf{y}^0]$} 
\FOR{each $t \in [0, 1,..., T]$}
\STATE generate non-negative matrices $W^t_{in}$, $W^t_{out}$

\FOR{each $m \in [1, ..., d]$}
\STATE construct a row-stochastic $A^t_m$  and a column-stochastic $B^t_m$ according to \eqref{eq:normA} and \eqref{eq:normB}

\STATE construct $\bar{M}^t_m$ according to \eqref{matrixdefbar}
\FOR{each $i \in \left\{1, ..., 2n \right\}$}
\STATE 
\begin{equation*}
\begin{aligned}
z_{im}^{t+1} & = \sum_{j=1}^{2n}[\bar{M}^t_m]_{ij} [Q(\z_{j}^t)]_m + \mathbbm{1}_{\left\{t\mod \mathcal{B} = \mathcal{B}-1\right\}} \epsilon [F]_{ij} z_{jm}^{\mathcal{B} \lfloor t/\mathcal{B} \rfloor}
\end{aligned}
\end{equation*}
\ENDFOR
\ENDFOR
\ENDFOR

\end{algorithmic}
\end{algorithm}


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
The proof of Lemma \ref{lemma0} is in Appendix \ref{app:A}.
 
\begin{remark}
In Appendix \ref{app:C}, we establish that under the assumption of connected random graphs following Erd{\"o}s–Rényi generative model \cite{erdos1959random}, $\sigma$ is inversely related to the square root of  the compression rate, $\sqrt{k/d}$. Therefore, as the rate of sparsification increases, so does $\sigma$; this, in turn, reduces the convergence rate.
\end{remark}

Lemma \ref{lemma0} implies that the product of mixing matrices converges to its limit % in \eqref{eq:limit} 
at a geometric rate; this intermediate result can be used to establish the geometric convergence rate of Algorithm \ref{alg:A} for the average consensus problem.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem1}
Suppose Assumptions \ref{assumption0} and \ref{assumption2} hold, and instate the notations and hypotheses above. Then, there exist $\sigma \in (0, 1)$ and $\Gamma = \sqrt{2nd}$ such that the following statements hold.
\begin{enumerate}[(a)]
%    \item For $1 \leq i \leq n$ and $t = kT - 1$, 
%    \begin{equation}
%    \|\mathbf{z}_i^t-\mathbf{\Bar{z}}\| \leq \Gamma \sigma^{k} \sum_{j=1}^{2n}\sum_{m=1}^d |z^0_{jm}|,
%    \end{equation}
%    where $\mathbf{\Bar{z}}=\frac{1}{n}\sum_{i=1}^n \mathbf{x}_i^0 +\frac{1}{n}\sum_{i=1}^n \mathbf{y}_i^0$;
    \item For $1 \leq i \leq n$ and $t = k\mathcal{B} - 1 + t'$, where $t' = 0, \cdots, \mathcal{B}-1$,
    \begin{equation}
    \|\mathbf{z}_i^t-\mathbf{\Bar{z}}\| \leq \Gamma \sigma^{k} \sum_{j=1}^{2n}\sum_{m=1}^d |z^0_{jm}|,
    \end{equation}
    \begin{equation}
    \|\mathbf{z}_i^t-\mathbf{\Bar{z}}\| \leq \Gamma (\sigma^{1/\mathcal{B}})^{t-(t'-1) } \sum_{j=1}^{2n}\sum_{m=1}^d |z^0_{jm}|,
    \end{equation}
    where $\mathbf{\Bar{z}}=\frac{1}{n}\sum_{i=1}^n \mathbf{x}_i^0 +\frac{1}{n}\sum_{i=1}^n \mathbf{y}_i^0$;
    \item 
    For $1+n \leq i \leq 2n$ and $t = k\mathcal{B} - 1 + t'$, where $t' = 0, \cdots, \mathcal{B}-1$, 
    \begin{equation}
    \|\mathbf{z}_i^t\| \leq \Gamma \sigma^{k}\sum_{j=1}^{2n}\sum_{m=1}^d |z^0_{jm}|.
    \end{equation}
    \begin{equation}
    \|\mathbf{z}_i^t\| \leq \Gamma (\sigma^{1/\mathcal{B}})^{t-(t'-1) }\sum_{j=1}^{2n}\sum_{m=1}^d |z^0_{jm}|.
    \end{equation}
    
\end{enumerate}
\end{theorem}

Based on the definition of $\z_i^t$ in \eqref{eq:zdef}, $\x_i^t$ is relevant to (a) and $\y_i^t$ is relevant to (b). In particular, the first part of Theorem \ref{theorem1} implies that the local parameters $\x_i^t$ converge at a linear rate to the average of the initial values $\Bar{\mathbf{z}}$. The second part of the theorem establishes that the auxiliary variables defined in order to handle directed communication in the network converge linearly to zero. Therefore, by initializing $\mathbf{y}_i^0=\mathbf{0}$, we can guarantee the consensus property and the linear convergence rate of Algorithm \ref{alg:A}. The proof of Theorem \ref{theorem1} can be found in Appendix \ref{app:A}.


